$f_B$ and $f_{B_s}$ using NRQCD

This talk summarizes the quenched calculation of $f_B$ and $f_{B_s}$ presented in hep-lat/9801038. The heavy quark is simulated using an $O(1/M^2)$ improved NRQCD action, and the tadpole improved clover action is used for the light quarks. The axial current includes the $O(1/M)$ corrections in one-loop perturbation theory and the $O(1/M^2)$ ones at tree-level. We discuss the various systematic effects and consistency checks made in the calculation.

==> Makefile <==
# %auto-ignore
MAINFILE=  fB.tex

TEXFILES=  
AXISFILES= 
FIGFILES=  
PSFILES=   
#########################################################################
# special rules if any

#########################################################################
#									#
#                 NO USER SERVICEABLE PARTS BELOW !!!                   #
# 									#
#########################################################################


# List of all the sources
SOURCES= Makefile ${MAINFILE} ${TEXFILES} ${AXISFILES} ${FIGFILES} ${PSFILES}

# List of all postscript figures to be included.
PSINCLUSIONS= ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps} ${PSFILES}

# what is to be made by default
all: ${MAINFILE:.tex=.ps}

# re-dvips if any of these change
${MAINFILE:.tex=.ps}: ${MAINFILE:.tex=.dvi} ${PSINCLUSIONS}

# re-latex if any of these change
${MAINFILE:.tex=.dvi}: ${MAIN} ${TEXFILES} ${PSINCLUSIONS}

# Never try to `make' any of the sources
${SOURCES}:;

# The rest of them do not have any `extra' dependencies, i.e. a.x depends 
# obviously depends on a.y if a.x is to be created from a.y.

.PHONY: clean realclean
# clean removes ~ aux log and tmp files
clean:
	rm -f *~ *.aux *.log *.tmp
# real clean removes everything but sources and final products
realclean: clean
	rm -f ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps}

########################################################################
# General rules of how to build something from something else.
.SUFFIXES: .ps .dvi .tex .ax .xy .fig

# If .fig exists that is how to create ps.
%.ps: %.fig
	fig2dev -L ps $< > $@

# If .ax or .xy exist, that is the source of the .ps file
%.ps: %.ax
	xyplot $< | epsplot > $@.tmp
	sed -e "/%%BoundingBox: /d" -e '1a\
	'"`psbbox $@.tmp`" $@.tmp > $@ 
	rm -f $@.tmp
%.ps: %.xy
	xyplot $< | epsplot > $@.tmp
	sed -e "/%%BoundingBox: /d" -e '1a\
	'"`psbbox $@.tmp`" $@.tmp > $@ 
	rm -f $@.tmp

# else look for a dvi file.
%.ps: %.dvi
	dvips -z -o $@ $<


# dvi is always created from tex.
%.dvi: %.tex
	latex $<
	if grep -i -q rerun ${<:.tex=.log} ; then latex $<; fi
##################################################################

submission: ${SOURCES} ${PSINCLUSIONS}
	(echo "."; \
	 echo "${SOURCES} ${PSINCLUSIONS}" ; \
	 echo "submission") | uufiles -gz -9

